A Course on Elementary Probability Theory

This book introduces to the theory of probabilities from the beginning. Assuming that the reader possesses the normal mathematical level acquired at the end of the secondary school, we aim to equip him with a solid basis in probability theory. The theory is preceded by a general chapter on counting methods. Then, the theory of probabilities is presented in a discrete framework. Two objectives are sought. The first is to give the reader the ability to solve a large number of problems related to probability theory, including application problems in a variety of disciplines. The second was to prepare the reader before he approached the manual on the mathematical foundations of probability theory. In this book, the reader will concentrate more on mathematical concepts, while in the present text, experimental frameworks are mostly found. If both objectives are met, the reader will have already acquired a definitive experience in problem-solving ability with the tools of probability theory and at the same time he is ready to move on to a theoretical course on probability theory based on the theory of measurement and integration. The book ends with a chapter that allows the reader to begin an intermediate course in mathematical statistics.

==> preface_ed1_en.tex <==
\chapter*{Preface of the first edition 2016}

The current series of Probability Theory and Statistics are based on two {introductory  books for beginners} : A Course of Elementary probability Theory and A course on Descriptive Statistics.\\  

\noindent All the more or less advanced probability courses are preceded by this one. We strongly recommend to not skip it. It has the tremendous advantage to make feel the reader the essence of probability theory by using extensively random experiences. The mathematical concepts come only after a complete description of a random experience.\\

\noindent  This book introduces to the theory of probabilities from the beginning. Assuming that the reader possesses the normal mathematical level acquired at the end of the secondary school, we aim to equip him with a solid basis in probability theory. The theory is preceded by a general chapter on counting methods. Then, the theory of probabilities is presented in a discrete framework.\\

\noindent Two objectives are sought. The first is to give the reader the ability to solve a large number of problems related to probability theory, including application problems in a variety of disciplines. The second was to prepare the reader before he approached the textbook on the mathematical foundations of probability theory. In this book, the reader will concentrate more on mathematical concepts, while in the present text, experimental frameworks are mostly found. If both objectives are met, the reader will have already acquired a definitive experience in problem-solving ability with the tools of probability theory and at the same time he is ready to move on to a theoretical course on probability theory based on the theory of measurement and integration.\\

\noindent The book ends with a chapter that allows the reader to begin an intermediate course in mathematical statistics.

\noindent I wish you a pleasant reading and hope receiving your feedback.\\

\noindent To my late and beloved sister Khady Kane Lo(1953-  ).\\

\noindent Saint-Louis, Calgary, Abuja, Bamako, Ouagadougou, 2017. 
  
\newpage
\noindent \huge \textbf{Preliminary Remarks and Notations}.\\

\Large
 
\bigskip \bigskip
\noindent \textbf{WARNINGS}\\

\noindent \textbf{(1)} \\

\noindent \textbf{(2)} \\

\endinput

==> preface_gen_en.tex <==
\chapter*{General Preface}



\noindent \textbf{This textbook} part of a series whose ambition is to cover broad part of Probability Theory and Statistics.  These textbooks are intended to help learners and readers, both of of all levels, to train themselves.\\

\noindent As well, they may constitute helpful documents for professors and teachers for both courses and exercises.  For more ambitious  people, they are only starting points towards more advanced and personalized books. So, these texts are kindly put at the disposal of professors and learners.


\bigskip \noindent \textbf{Our textbooks are classified into categories}.\\

\noindent \textbf{A series of introductory  books for beginners}. Books of this series are usually accessible to student of first year in 
universities. They do not require advanced mathematics.  Books on elementary probability theory and descriptive statistics are to be put in that category. Books of that kind are usually introductions to more advanced and mathematical versions of the same theory. The first prepare the applications of the second.\\

\noindent \textbf{A series of books oriented to applications}. Students or researchers in very related disciplines  such as Health studies, Hydrology, Finance, Economics, etc.  may be in need of Probability Theory or Statistics. They are not interested by these disciplines  by themselves.  Rather, the need to apply their findings as tools to solve their specific problems. So adapted books on Probability Theory and Statistics may be composed to on the applications of such fields. A perfect example concerns the need of mathematical statistics for economists who do not necessarily have a good background in Measure Theory.\\


\noindent \textbf{A series of specialized books on Probability theory and Statistics of high level}. This series begin with a book on Measure Theory, its counterpart of probability theory, and an introductory book on topology. On that basis, we will have, as much as possible,  a coherent presentation of branches of Probability theory and Statistics. We will try  to have a self-contained, as much as possible, so that anything we need will be in the series.\\


\noindent Finally, \textbf{research monographs} close this architecture. The architecture should be so large and deep that the readers of monographs booklets will find all needed theories and inputs in it.\\



\bigskip \noindent We conclude by saying that, with  only an undergraduate level, the reader will  open the door of anything in Probability theory and statistics with \textbf{Measure Theory and integration}. Once this course validated, eventually combined with two solid courses on topology and functional analysis, he will have all the means to get specialized in any branch in these disciplines.\\

\bigskip \noindent Our collaborators and former students are invited to make live this trend and to develop it so  that  the center of Saint-Louis becomes or continues to be a re-known mathematical school, especially in Probability Theory and Statistics.


\endinput
